Predictive Process Model Monitoring using Recurrent Neural Networks

The field of predictive process monitoring focuses on case-level models to predict a single specific outcome such as a particular objective, (remaining) time, or next activity/remaining sequence. Recently, a longer-horizon, model-wide approach has been proposed in the form of process model forecasting, which predicts the future state of a whole process model through the forecasting of all activity-to-activity relations at once using time series forecasting. This paper introduces the concept of \emph{predictive process model monitoring} which sits in the middle of both predictive process monitoring and process model forecasting. Concretely, by modelling a process model as a set of constraints being present between activities over time, we can capture more detailed information between activities compared to process model forecasting, while being compatible with typical predictive process monitoring objectives which are often expressed in the same language as these constraints. To achieve this, Processes-As-Movies (PAM) is introduced, i.e., a novel technique capable of jointly mining and predicting declarative process constraints between activities in various windows of a process' execution. PAM predicts what declarative rules hold for a trace (objective-based), which also supports the prediction of all constraints together as a process model (model-based). Various recurrent neural network topologies inspired by video analysis tailored to temporal high-dimensional input are used to model the process model evolution with windows as time steps, including encoder-decoder long short-term memory networks, and convolutional long short-term memory networks. Results obtained over real-life event logs show that these topologies are effective in terms of predictive accuracy and precision.

==> tab-fixedlength-conv.tex <==
\begin{figure}  
  \centering    
  \begin{subfigure}[b]{\textwidth}
  	\includegraphics[width=1.0\textwidth]{img/CONVbpi122.png}
  	\caption{BPI 12, 2 windows.}
  	\label{fig:tiger}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth}
	\includegraphics[width=1.0\textwidth]{img/CONVbpi125.png}
	\caption{BPI 12, 5 windows.}
	\label{fig:tiger}
\end{subfigure}
  \begin{subfigure}[b]{\textwidth}
	\includegraphics[width=1.0\textwidth]{img/CONVbpi1210.png}
	\caption{BPI 12, 10 windows.}
	\label{fig:tiger}
\end{subfigure}
  \begin{subfigure}[b]{\textwidth}
	\includegraphics[width=1.0\textwidth]{img/CONVbpi172.png}
	\caption{BPI 17, 2 windows.}
	\label{fig:tiger}
\end{subfigure}
  \begin{subfigure}[b]{\textwidth}
	\includegraphics[width=1.0\textwidth]{img/CONVbpi175.png}
	\caption{BPI 17, 5 windows.}
	\label{fig:tiger}
\end{subfigure}
  \begin{subfigure}[b]{\textwidth}
	\includegraphics[width=1.0\textwidth]{img/CONVbpi1710.png}
	\caption{BPI 17, 10 windows.}
	\label{fig:tiger}
\end{subfigure}
   \caption{CONVLSTMs, fixed number of windows. Kernel size on the x-axis, different lines per filter size.}
\end{figure}

==> tab-fixedlength-de.tex <==
\begin{figure}  
  \centering    
  \begin{subfigure}[b]{\textwidth}
  	\includegraphics[width=1.0\textwidth]{img/DEbpi12.png}
  	\caption{BPI 12.}
  	\label{fig:tiger}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth}
	\includegraphics[width=1.0\textwidth]{img/DEbpi17.png}
	\caption{BPI 17.}
	\label{fig:tiger}
\end{subfigure}
   \caption{Encoder-decoder LSTMs, fixed number of windows. Number of latent dimensions on the x-axis, different lines per number of LSTM layers.}
\end{figure}

==> tab-fixedwindow-conv.tex <==
\begin{figure}  
  \centering    
  \begin{subfigure}[b]{\textwidth}
  	\includegraphics[width=1.0\textwidth]{img/CONVbpi12210u20.png}
  	\caption{6-10 windows.}
  	\label{fig:tiger}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth}
	\includegraphics[width=1.0\textwidth]{img/CONVbpi12220u30.png}
	\caption{11-15 windows.}
	\label{fig:tiger}
\end{subfigure}
  \begin{subfigure}[b]{\textwidth}
	\includegraphics[width=1.0\textwidth]{img/CONVbpi12230u40.png}
	\caption{16-20 windows.}
	\label{fig:tiger}
\end{subfigure}
  \begin{subfigure}[b]{\textwidth}
	\includegraphics[width=1.0\textwidth]{img/CONVbpi12240u50.png}
	\caption{21-25 windows.}
	\label{fig:tiger}
\end{subfigure}
  \begin{subfigure}[b]{\textwidth}
	\includegraphics[width=1.0\textwidth]{img/CONVbpi12250u60.png}
	\caption{26-30 windows.}
	\label{fig:tiger}
\end{subfigure}
   \caption{CONVLSTMs, BPI 12, window size 2. Kernel size on the x-axis, different lines per filter size.}
\end{figure}

\begin{figure}  
	\centering    
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi12510u20.png}
		\caption{3-4 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi12520u30.png}
		\caption{5-6 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi12530u40.png}
		\caption{7-8 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi12540u50.png}
		\caption{9-10 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi12550u60.png}
		\caption{11-12 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\caption{CONVLSTMs, BPI 12, window size 5. Kernel size on the x-axis, different lines per filter size.}
\end{figure}

\begin{figure}  
	\centering    
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi121010u20.png}
		\caption{2 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi121020u30.png}
		\caption{3 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi121030u40.png}
		\caption{4 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi121040u50.png}
		\caption{5 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi121050u60.png}
		\caption{6 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\caption{CONVLSTMs, BPI 12, window size 10. Kernel size on the x-axis, different lines per filter size.}
\end{figure}

\begin{figure}  
	\centering    
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi17210u20.png}
		\caption{6-10 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi17220u30.png}
		\caption{11-15 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi17230u40.png}
		\caption{16-20 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi17240u50.png}
		\caption{21-25 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi17250u60.png}
		\caption{26-30 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\caption{CONVLSTMs, BPI 17, window size 2. Kernel size on the x-axis, different lines per filter size.}
\end{figure}

\begin{figure}  
	\centering    
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi17510u20.png}
		\caption{3-4 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi17520u30.png}
		\caption{5-6 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi17530u40.png}
		\caption{7-8 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi17540u50.png}
		\caption{9-10 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi17550u60.png}
		\caption{11-12 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\caption{CONVLSTMs, BPI 17, window size 5. Kernel size on the x-axis, different lines per filter size.}
\end{figure}

\begin{figure}  
	\centering    
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi171010u20.png}
		\caption{2 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi171020u30.png}
		\caption{3 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi171030u40.png}
		\caption{4 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi171040u50.png}
		\caption{5 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=1.0\textwidth]{img/CONVbpi171050u60.png}
		\caption{6 windows.}
		\label{fig:tiger}
	\end{subfigure}
	\caption{CONVLSTMs, BPI 17, window size 10. Kernel size on the x-axis, different lines per filter size.}
\end{figure}

==> tab-fixedwindow-de.tex <==
\begin{figure}  
  \centering 
   \begin{subfigure}[b]{\textwidth}
 	\includegraphics[width=1.0\textwidth]{img/DEbpi122.png}
 	\caption{BPI 12, window size 2}
 	\label{fig:tiger}
 \end{subfigure}   
  \begin{subfigure}[b]{\textwidth}
  	\includegraphics[width=1.0\textwidth]{img/DEbpi125.png}
  	\caption{BPI 12, window size 5}
  	\label{fig:tiger}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth}
	\includegraphics[width=1.0\textwidth]{img/DEbpi1210.png}
	\caption{BPI 12, window size 10}
	\label{fig:tiger}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
	\includegraphics[width=1.0\textwidth]{img/DEbpi172.png}
	\caption{BPI 17, window size 2}
	\label{fig:tiger}
\end{subfigure}
 \begin{subfigure}[b]{\textwidth}
	\includegraphics[width=1.0\textwidth]{img/DEbpi175.png}
	\caption{BPI 17, window size 5}
	\label{fig:tiger}
\end{subfigure}
  \begin{subfigure}[b]{\textwidth}
	\includegraphics[width=1.0\textwidth]{img/DEbpi1710.png}
	\caption{BPI 17, window size 10}
	\label{fig:tiger}
\end{subfigure}
   \caption{Encoder-decoder LSTMs, fixed window size. Number of latent dimensions on the x-axis, different lines per number of LSTM layers.}
\end{figure}

==> tab-res-fixedwinsize.tex <==
\begin{table}
	\centering
	\resizebox{\textwidth}{!}{
		
% Table generated by Excel2LaTeX from sheet 'Fixed window length NoQuart'
\begin{tabular}{|c|c|l|r|r|r|r|r|r|r|r|r|r|}
	\cline{4-13}\multicolumn{1}{r}{} & \multicolumn{1}{r}{} &       & \multicolumn{5}{c|}{\textbf{Convolutional LSTMs}} & \multicolumn{5}{c|}{\textbf{Encoder-decoder LSTMs}} \bigstrut\\
	\hline
	\multicolumn{1}{|l|}{\textbf{Event log}} & \multicolumn{1}{l|}{\textbf{\#Win.}} & \textbf{Metric} & \multicolumn{1}{c|}{\textbf{mean}} & \multicolumn{1}{c|}{\textbf{std}} & \multicolumn{1}{c|}{\textbf{min}} & \multicolumn{1}{c|}{\textbf{med}} & \multicolumn{1}{c|}{\textbf{max}} & \multicolumn{1}{c|}{\textbf{mean}} & \multicolumn{1}{c|}{\textbf{std}} & \multicolumn{1}{c|}{\textbf{min}} & \multicolumn{1}{c|}{\textbf{med}} & \multicolumn{1}{c|}{\textbf{max}} \bigstrut\\
	\hline
	\multirow{20}[40]{*}{\textbf{BPI 12 (2)}} & \multirow{4}[8]{*}{\textbf{6--10}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.973} & 0.034 & 0.799 & 0.985 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.992} & 0.574 & 0.369 & 0.005 & 0.737 & 0.982 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.997} & 0.015 & 0.91  & 1     & \textbf{1} & 0.669 & 0.233 & 0.49  & 0.5   & \textbf{1} \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.924} & 0.035 & 0.801 & 0.94  & \textbf{0.959} & 0.619 & 0.316 & 0.011 & 0.808 & 0.936 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 8.82  & 2.974 & 4.237 & 8.373 & 16.33 & 4.015 & 1.324 & 1.923 & 4.142 & 6.173 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{11--15}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.966} & 0.036 & 0.832 & 0.977 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.996} & 0.71  & 0.211 & 0.234 & 0.726 & 0.977 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.999} & 0.004 & 0.978 & 1     & \textbf{1} & 0.673 & 0.234 & 0.491 & 0.5   & 0.998 \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.916} & 0.042 & 0.817 & 0.921 & \textbf{0.97} & 0.782 & 0.125 & 0.392 & 0.831 & 0.922 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 29.167 & 36.894 & 8.638 & 19.424 & 230.284 & 8.876 & 2.674 & 4.715 & 9.178 & 13.645 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{16--20}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.934} & 0.064 & 0.629 & 0.955 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.973} & 0.649 & 0.15  & 0.303 & 0.685 & 0.961 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.994} & 0.014 & 0.923 & 0.999 & \textbf{1} & 0.531 & 0.125 & 0.496 & 0.5   & 0.999 \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.885} & 0.035 & 0.699 & 0.89  & \textbf{0.921} & 0.78  & 0.106 & 0.48  & 0.823 & 0.889 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 25.853 & 14.005 & 9.197 & 22.036 & 68.545 & 9.313 & 2.891 & 4.861 & 9.679 & 14.31 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{21--25}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.891} & 0.15  & 0.025 & 0.92  & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.948} & 0.657 & 0.086 & 0.459 & 0.698 & 0.724 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.993} & 0.032 & 0.804 & 0.999 & \textbf{1} & 0.5   & 0     & 0.5   & 0.5   & 0.5 \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.847} & 0.131 & 0.083 & 0.868 & \textbf{0.89} & 0.799 & 0.063 & 0.655 & 0.83  & 0.847 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 18.425 & 10.369 & 6.536 & 15.207 & 49.744 & 6.507 & 2.068 & 3.325 & 6.725 & 9.953 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{26--30}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.906} & 0.018 & 0.838 & 0.909 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.931} & 0.659 & 0.119 & 0.327 & 0.702 & 0.75 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.996} & 0.003 & 0.989 & 0.997 & \textbf{0.999} & 0.5   & 0     & 0.5   & 0.5   & 0.5 \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.867} & 0.008 & 0.855 & 0.867 & \textbf{0.885} & 0.801 & 0.088 & 0.54  & 0.832 & 0.862 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 43.557 & 191.57 & 4.037 & 9.574 & 1160.43 & 3.935 & 1.248 & 2.002 & 4.092 & 6.1 \bigstrut\\
	\hline
	\multirow{20}[40]{*}{\textbf{BPI 12 (5)}} & \multirow{4}[8]{*}{\textbf{3--4}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.941} & 0.016 & 0.853 & 0.943 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.953} & 0.877 & 0.121 & 0.564 & 0.918 & 0.948 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.999} & 0.001 & 0.992 & 0.999 & \textbf{1} & 0.973 & 0.06  & 0.817 & 0.997 & \textbf{1} \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.851} & 0.011 & 0.803 & 0.851 & \textbf{0.867} & 0.822 & 0.036 & 0.743 & 0.833 & 0.864 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 4.547 & 1.511 & 2.229 & 4.291 & 7.939 & 2.487 & 0.739 & 1.376 & 2.586 & 3.863 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{5--6}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.922} & 0.025 & 0.849 & 0.932 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.948} & 0.799 & 0.15  & 0.46  & 0.835 & 0.933 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.999} & 0.001 & 0.997 & 0.999 & \textbf{1} & 0.962 & 0.079 & 0.773 & 0.998 & 0.999 \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.828} & 0.025 & 0.768 & 0.838 & \textbf{0.858} & 0.755 & 0.059 & 0.667 & 0.747 & 0.834 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 11.44 & 5.602 & 4.454 & 9.68  & 28.208 & 5.078 & 1.607 & 2.475 & 5.163 & 8.016 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{7--8}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.873} & 0.076 & 0.665 & 0.909 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.936} & 0.795 & 0.108 & 0.507 & 0.798 & 0.899 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.996} & 0.005 & 0.976 & 0.998 & \textbf{0.999} & 0.974 & 0.066 & 0.781 & 0.997 & \textbf{0.999} \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.791} & 0.05  & 0.677 & 0.814 & \textbf{0.845} & 0.74  & 0.038 & 0.691 & 0.725 & 0.799 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 12.307 & 6.48  & 4.385 & 10.345 & 31.236 & 5.137 & 1.545 & 2.508 & 5.239 & 7.873 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{9--10}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.8} & 0.083 & 0.533 & 0.822 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.909} & 0.661 & 0.175 & 0.293 & 0.739 & 0.846 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.994} & 0.01  & 0.954 & 0.997 & \textbf{0.999} & 0.918 & 0.108 & 0.72  & 0.994 & 0.998 \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.729} & 0.052 & 0.599 & 0.738 & \textbf{0.818} & 0.668 & 0.05  & 0.528 & 0.682 & 0.746 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 8.76  & 4.661 & 3.064 & 7.311 & 22.387 & 3.518 & 1.083 & 1.778 & 3.609 & 5.575 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{11--12}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.73} & 0.051 & 0.511 & 0.743 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.798} & 0.61  & 0.149 & 0.239 & 0.693 & 0.768 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.988} & 0.026 & 0.848 & 0.995 & \textbf{0.997} & 0.907 & 0.117 & 0.715 & 0.992 & 0.996 \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.678} & 0.019 & 0.624 & 0.676 & \textbf{0.716} & 0.651 & 0.047 & 0.482 & 0.663 & 0.678 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 5.608 & 2.94  & 1.927 & 4.759 & 14.176 & 2.152 & 0.646 & 1.117 & 2.165 & 3.371 \bigstrut\\
	\hline
	\multirow{20}[40]{*}{\textbf{BPI 12 (10)}} & \multirow{4}[8]{*}{\textbf{2}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.922} & 0.016 & 0.887 & 0.923 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.957} & 0.858 & 0.184 & 0.377 & 0.926 & 0.947 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.998} & 0.002 & 0.989 & 0.999 & \textbf{0.999} & 0.965 & 0.09  & 0.728 & 0.998 & \textbf{0.999} \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.844} & 0.017 & 0.814 & 0.844 & \textbf{0.89} & 0.818 & 0.088 & 0.585 & 0.848 & 0.877 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 2.423 & 0.646 & 1.449 & 2.386 & 3.78  & 1.748 & 0.501 & 1.122 & 1.752 & 2.916 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{3}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.827} & 0.019 & 0.779 & 0.832 & 0.854 & 0.787 & 0.124 & 0.342 & 0.814 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.858} \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.997} & 0.001 & 0.994 & 0.997 & 0.998 & 0.979 & 0.073 & 0.705 & 0.997 & \textbf{0.999} \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.736} & 0.019 & 0.695 & 0.738 & \textbf{0.768} & 0.712 & 0.054 & 0.548 & 0.726 & 0.764 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 5.585 & 2.288 & 2.679 & 5.293 & 12.431 & 3.404 & 1.174 & 1.815 & 3.57  & 5.906 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{4}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.821} & 0.035 & 0.711 & 0.831 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.868} & 0.727 & 0.172 & 0.261 & 0.802 & 0.851 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.997} & 0.002 & 0.99  & 0.997 & \textbf{0.999} & 0.96  & 0.1   & 0.698 & 0.997 & 0.998 \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.725} & 0.029 & 0.637 & 0.733 & \textbf{0.769} & 0.67  & 0.076 & 0.492 & 0.704 & 0.748 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 6.08  & 2.789 & 2.567 & 5.338 & 14.182 & 3.253 & 1.05  & 1.761 & 3.369 & 5.269 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{5}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.758} & 0.047 & 0.652 & 0.777 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.819} & 0.681 & 0.146 & 0.166 & 0.709 & 0.783 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.994} & 0.003 & 0.987 & 0.995 & \textbf{0.997} & 0.974 & 0.082 & 0.665 & 0.995 & \textbf{0.997} \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.671} & 0.037 & 0.581 & 0.685 & \textbf{0.721} & 0.614 & 0.071 & 0.395 & 0.622 & 0.691 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 4.352 & 2.056 & 1.733 & 3.795 & 10.35 & 2.206 & 0.715 & 1.064 & 2.287 & 3.546 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{6}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.688} & 0.045 & 0.597 & 0.692 & 0.772 & 0.625 & 0.165 & 0.189 & 0.665 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.779} \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.991} & 0.004 & 0.978 & 0.993 & 0.995 & 0.951 & 0.11  & 0.653 & 0.993 & \textbf{0.997} \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.616} & 0.037 & 0.555 & 0.614 & \textbf{0.689} & 0.583 & 0.065 & 0.406 & 0.593 & 0.667 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 2.898 & 1.424 & 1.131 & 2.495 & 7.01  & 1.356 & 0.412 & 0.692 & 1.368 & 2.144 \bigstrut\\
	\hline
\end{tabular}%
	
	}
	\caption{An overview of the performance of both neural network approaches for a fixed window size trained over different subsets of the data containing different numbers of windows. The highest average and maximum precision (AP) is indicated in grey, the other metrics in bold.}
	\label{tab:fixedwinsize12}
\end{table}

==> tab-res-fixedwinsize17.tex <==
\begin{table}
	\centering
	\resizebox{\textwidth}{!}{
		
% Table generated by Excel2LaTeX from sheet 'Fixed window length NoQuart'
\begin{tabular}{|c|c|l|r|r|r|r|r|r|r|r|r|r|}
	\cline{4-13}\multicolumn{1}{r}{} & \multicolumn{1}{r}{} &       & \multicolumn{5}{c|}{\textbf{Convolutional LSTMs}} & \multicolumn{5}{c|}{\textbf{Encoder-decoder LSTMs}} \bigstrut\\
	\hline
	\multicolumn{1}{|l|}{\textbf{Event log}} & \multicolumn{1}{l|}{\textbf{\#Win.}} & \textbf{Metric} & \multicolumn{1}{c|}{\textbf{mean}} & \multicolumn{1}{c|}{\textbf{std}} & \multicolumn{1}{c|}{\textbf{min}} & \multicolumn{1}{c|}{\textbf{med}} & \multicolumn{1}{c|}{\textbf{max}} & \multicolumn{1}{c|}{\textbf{mean}} & \multicolumn{1}{c|}{\textbf{std}} & \multicolumn{1}{c|}{\textbf{min}} & \multicolumn{1}{c|}{\textbf{med}} & \multicolumn{1}{c|}{\textbf{max}} \bigstrut\\
	\hline
	\multirow{20}[40]{*}{\textbf{BPI 17 (2)}} & \multirow{4}[8]{*}{\textbf{6--10}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.96} & 0.105 & 0.559 & 0.997 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{1} & 0.819 & 0.306 & 0.109 & 0.992 & 0.999 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.964} & 0.122 & 0.463 & 0.998 & \textbf{1} & 0.842 & 0.238 & 0.499 & 0.995 & \textbf{1} \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.959} & 0.086 & 0.578 & 0.988 & \textbf{0.997} & 0.851 & 0.257 & 0.191 & 0.975 & 0.993 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 16.732 & 7.016 & 7.137 & 16.039 & 36.557 & 7.216 & 2.259 & 3.629 & 7.483 & 11.189 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{11--15}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.963} & 0.076 & 0.778 & 0.998 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{1} & 0.724 & 0.208 & 0.301 & 0.703 & 0.999 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.981} & 0.04  & 0.886 & 1     & \textbf{1} & 0.641 & 0.222 & 0.499 & 0.5   & 0.998 \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.971} & 0.046 & 0.862 & 0.992 & \textbf{0.998} & 0.824 & 0.134 & 0.484 & 0.834 & 0.995 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 141.21 & 78.014 & 51.816 & 117.24 & 376.791 & 56.018 & 12.31 & 40.244 & 55.498 & 81.215 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{16--20}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.979} & 0.047 & 0.813 & 0.997 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{1} & 0.715 & 0.226 & 0.168 & 0.697 & 0.998 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.993} & 0.023 & 0.906 & 1     & \textbf{1} & 0.654 & 0.237 & 0.495 & 0.5   & 0.998 \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.967} & 0.044 & 0.859 & 0.982 & \textbf{0.997} & 0.803 & 0.144 & 0.371 & 0.83  & 0.986 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 130.98 & 72.696 & 45.208 & 107.83 & 349.506 & 47.382 & 14.18 & 25.15 & 49.617 & 71.148 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{21--25}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.949} & 0.168 & 0.032 & 0.997 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{1} & 0.645 & 0.168 & 0.255 & 0.707 & 0.869 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.981} & 0.079 & 0.546 & 1     & \textbf{1} & 0.5   & 0.001 & 0.496 & 0.5   & 0.5 \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.934} & 0.152 & 0.122 & 0.98  & \textbf{0.996} & 0.779 & 0.135 & 0.41  & 0.835 & 0.885 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 120.95 & 68.359 & 40.925 & 100.15 & 325.313 & 42.942 & 13.49 & 22.604 & 43.995 & 65.154 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{26--30}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.945} & 0.161 & 0.028 & 0.98  & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.994} & 0.673 & 0.134 & 0.325 & 0.734 & 0.759 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.97} & 0.123 & 0.402 & 1     & \textbf{1} & 0.5   & 0     & 0.5   & 0.5   & 0.5 \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.913} & 0.142 & 0.111 & 0.947 & \textbf{0.966} & 0.807 & 0.1   & 0.533 & 0.854 & 0.868 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 87.738 & 49.534 & 28.326 & 71.171 & 233.279 & 29.611 & 8.965 & 15.747 & 30.777 & 45.045 \bigstrut\\
	\hline
	\multirow{20}[40]{*}{\textbf{BPI 17 (5)}} & \multirow{4}[8]{*}{\textbf{3--4}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.946} & 0.117 & 0.52  & 0.984 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.992} & 0.945 & 0.16  & 0.343 & 0.984 & 0.991 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & 0.977 & 0.067 & 0.74  & 0.999 & \textbf{1} & \textbf{0.981} & 0.072 & 0.711 & 0.999 & \textbf{1} \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.938} & 0.073 & 0.668 & 0.96  & \textbf{0.975} & 0.934 & 0.102 & 0.554 & 0.961 & 0.974 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 7.944 & 2.968 & 3.803 & 7.434 & 16.159 & 4.318 & 1.408 & 2.232 & 4.377 & 6.791 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{5--6}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.972} & 0.063 & 0.616 & 0.987 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.991} & 0.913 & 0.184 & 0.402 & 0.983 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.991} \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.992} & 0.034 & 0.802 & 1     & \textbf{1} & 0.975 & 0.066 & 0.803 & 1     & \textbf{1} \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.937} & 0.035 & 0.751 & 0.946 & \textbf{0.955} & 0.898 & 0.095 & 0.632 & 0.935 & \textbf{0.955} \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 65.707 & 34.593 & 23.683 & 54.083 & 165.441 & 28.821 & 7.956 & 14.266 & 29.037 & 44.884 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{7--8}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.962} & 0.032 & 0.818 & 0.972 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.981} & 0.813 & 0.214 & 0.362 & 0.903 & 0.973 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.998} & 0.005 & 0.97  & 1     & \textbf{1} & 0.947 & 0.093 & 0.775 & 0.999 & 1 \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.899} & 0.036 & 0.748 & 0.908 & \textbf{0.923} & 0.8   & 0.097 & 0.598 & 0.812 & 0.909 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 62.294 & 32.61 & 22.007 & 52.266 & 157.082 & 24.881 & 7.39  & 12.399 & 26.382 & 37.663 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{9--10}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.927} & 0.072 & 0.692 & 0.959 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.98} & 0.7   & 0.238 & 0.251 & 0.807 & 0.964 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.992} & 0.03  & 0.851 & 0.999 & \textbf{1} & 0.905 & 0.107 & 0.763 & 0.964 & \textbf{1} \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.87} & 0.066 & 0.7   & 0.897 & \textbf{0.93} & 0.732 & 0.106 & 0.498 & 0.741 & 0.897 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 57.955 & 31.685 & 19.484 & 48.078 & 146.974 & 22.138 & 5.661 & 12.16 & 22.631 & 33.098 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{11--12}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.891} & 0.154 & 0.071 & 0.946 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.975} & 0.637 & 0.254 & 0.167 & 0.541 & 0.966 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.984} & 0.059 & 0.661 & 0.999 & \textbf{1} & 0.881 & 0.107 & 0.763 & 0.802 & \textbf{1} \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.83} & 0.134 & 0.149 & 0.882 & \textbf{0.924} & 0.715 & 0.123 & 0.392 & 0.719 & 0.898 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 39.968 & 21.802 & 13.066 & 32.77 & 102.656 & 14.626 & 4.393 & 7.361 & 15.037 & 22.494 \bigstrut\\
	\hline
	\multirow{20}[40]{*}{\textbf{BPI 17 (10)}} & \multirow{4}[8]{*}{\textbf{2}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.979} & 0.005 & 0.968 & 0.979 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.989} & 0.956 & 0.073 & 0.769 & 0.982 & 0.988 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.999} & 0     & 0.998 & 0.999 & \textbf{1} & 0.988 & 0.031 & 0.908 & 0.999 & \textbf{1} \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.952} & 0.008 & 0.935 & 0.951 & 0.966 & 0.945 & 0.029 & 0.874 & 0.953 & \textbf{0.97} \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 4.299 & 1.227 & 2.469 & 4.165 & 7.444 & 2.957 & 0.878 & 1.754 & 2.985 & 4.751 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{3}} & \textbf{AP} & 0.921 & 0.015 & 0.884 & 0.926 & 0.938 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.93} & 0.007 & 0.913 & 0.932 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.939} \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & 0.998 & 0.004 & 0.977 & 0.999 & \textbf{0.999} & \textbf{0.999} & 0.001 & 0.995 & 0.999 & \textbf{0.999} \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & 0.849 & 0.013 & 0.822 & 0.847 & \textbf{0.869} & \textbf{0.859} & 0.007 & 0.842 & 0.86  & 0.868 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 32.042 & 13.985 & 14.555 & 29.309 & 73.366 & 19.018 & 6.513 & 9.618 & 19.416 & 34.132 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{4}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.9} & 0.017 & 0.854 & 0.907 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.92} & 0.859 & 0.124 & 0.4   & 0.895 & 0.914 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.999} & 0.001 & 0.997 & 0.999 & \textbf{0.999} & 0.982 & 0.065 & 0.738 & 0.999 & \textbf{0.999} \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.805} & 0.014 & 0.772 & 0.808 & \textbf{0.822} & 0.78  & 0.051 & 0.606 & 0.797 & \textbf{0.822} \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 29.948 & 14.221 & 12.292 & 26.284 & 71.597 & 15.735 & 5.514 & 8.166 & 16.474 & 27.556 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{5}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.9} & 0.03  & 0.754 & 0.906 & \textbf{0.924} & 0.833 & 0.145 & 0.326 & 0.892 & 0.913 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.997} & 0.007 & 0.954 & 0.999 & \textbf{0.999} & 0.982 & 0.066 & 0.734 & 0.998 & \textbf{0.999} \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.817} & 0.026 & 0.7   & 0.821 & \textbf{0.84} & 0.763 & 0.077 & 0.558 & 0.8   & 0.829 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 27.997 & 13.784 & 10.725 & 23.641 & 67.197 & 13.343 & 4.629 & 6.21  & 13.464 & 22.833 \bigstrut\\
	\cline{2-13}      & \multirow{4}[8]{*}{\textbf{6}} & \textbf{AP} & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.897} & 0.02  & 0.836 & 0.904 & \cellcolor[rgb]{ .906,  .902,  .902}\textbf{0.922} & 0.8   & 0.181 & 0.147 & 0.83  & 0.908 \bigstrut\\
	\cline{3-13}      &       & \textbf{AUC} & \textbf{0.998} & 0.001 & 0.996 & 0.998 & \textbf{0.999} & 0.981 & 0.067 & 0.73  & 0.998 & \textbf{0.999} \bigstrut\\
	\cline{3-13}      &       & \textbf{F--score} & \textbf{0.821} & 0.02  & 0.765 & 0.826 & \textbf{0.851} & 0.73  & 0.109 & 0.372 & 0.738 & 0.826 \bigstrut\\
	\cline{3-13}      &       & \textbf{Time} & 20.053 & 10.388 & 7.425 & 16.488 & 50.366 & 8.973 & 2.936 & 4.414 & 9.092 & 14.846 \bigstrut\\
	\hline
\end{tabular}%

	
	}
	\caption{An overview of the performance of both neural network approaches for a fixed window size trained over different subsets of the 2017 BPI Challenge data containing different numbers of windows. The highest average and maximum precision AP is indicated in grey, the other metrics in bold.}
	\label{tab:fixedwinsize17}
\end{table}
